Action Graphs: Weakly-supervised Action Localization with Graph Convolution Networks

We present a method for weakly-supervised action localization based on graph convolutions. In order to find and classify video time segments that correspond to relevant action classes, a system must be able to both identify discriminative time segments in each video, and identify the full extent of each action. Achieving this with weak video level labels requires the system to use similarity and dissimilarity between moments across videos in the training data to understand both how an action appears, as well as the sub-actions that comprise the action's full extent. However, current methods do not make explicit use of similarity between video moments to inform the localization and classification predictions. We present a novel method that uses graph convolutions to explicitly model similarity between video moments. Our method utilizes similarity graphs that encode appearance and motion, and pushes the state of the art on THUMOS '14, ActivityNet 1.2, and Charades for weakly supervised action localization.

==> latex/figs/flow_fig.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/flow_fig_fig.pdf}
    \caption{Pipeline: Pretrained features of $d$ dimension are extracted for each time segment split into $l$ time segments. An appearance similarity function $\phi$ is learned on the video and used to train a graph convolution layer. Both $\phi$ and the output of the graph layer are connected to linear classifiers to get the classification probability across $n_c$ classes for each time segment. Both predictions are supervised with a multi instance learning loss for video level classification.}
    \vspace{-1em}
    \label{fig_pipeline}
\end{figure}

==> latex/figs/more_qual.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{latex/figs/more_qual_fig.pdf}
    \caption{\textbf{Additional qualitative results:} The groundtruth is in blue, and our detections are in green.}
    \label{fig_more_qual}
\end{figure*}
% for our model
